PG-RCNN: Semantic Surface Point Generation for 3D Object Detection

One of the main challenges in LiDAR-based 3D object detection is that the sensors often fail to capture the complete spatial information about the objects due to long distance and occlusion. Two-stage detectors with point cloud completion approaches tackle this problem by adding more points to the regions of interest (RoIs) with a pre-trained network. However, these methods generate dense point clouds of objects for all region proposals, assuming that objects always exist in the RoIs. This leads to the indiscriminate point generation for incorrect proposals as well. Motivated by this, we propose Point Generation R-CNN (PG-RCNN), a novel end-to-end detector that generates semantic surface points of foreground objects for accurate detection. Our method uses a jointly trained RoI point generation module to process the contextual information of RoIs and estimate the complete shape and displacement of foreground objects. For every generated point, PG-RCNN assigns a semantic feature that indicates the estimated foreground probability. Extensive experiments show that the point clouds generated by our method provide geometrically and semantically rich information for refining false positive and misaligned proposals. PG-RCNN achieves competitive performance on the KITTI benchmark, with significantly fewer parameters than state-of-the-art models. The code is available at https://github.com/quotation2520/PG-RCNN.

==> texts/tabel2_1.tex <==
\begin{table*}[ht!]
  \centering
  \caption{Performance comparison on the KITTI \textit{test} set with AP under 40 recall positions. Best performance value is in \textbf{bold}, second-best is \underline{underlined}.}
  \label{table:kitti_test}
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{l|c c c|c c c|c c c|c c c}
    \hline
    \multirow{2}{*}{Method} &
    \multicolumn{3}{c|}{Car 3D AP$_{R40}$} &
    \multicolumn{3}{c|}{Car BEV AP$_{R40}$} &
    % \multicolumn{3}{c|}{Ped. 3D AP_{R40}} &
    \multicolumn{3}{c|}{Cyc. 3D AP$_{R40}$} &
    \multicolumn{3}{c}{Cyc. BEV AP$_{R40}$} \\
    % \cline{2-10}
    & Easy & Mod. & Hard & Easy & Mod. & Hard & Easy & Mod. & Hard & Easy & Mod. & Hard  \\
    \hline
    SECOND \cite{second_yan} & 83.13 & 73.66 & 66.20 & 88.07 & 79.37 & 77.95 & 70.51 & 53.85 & 46.90 & 73.67 & 56.04 & 48.78 \\
    PointPillars \cite{pointpillars_lang} & 82.58 & 74.31 & 68.99 & 90.07 & 86.56 & 82.81 & 77.10 & 58.65 & 51.92 & 79.90 & 62.73 & 55.58 \\
    STD \cite{std_yang} & 87.95 & 79.71 & 75.09 & 94.74 & 89.19 & \underline{86.42} & 78.69& 61.59 & 55.30 & 81.36 & 67.23 & 59.35 \\
    3DSSD \cite{3dssd_yang} & 88.36 & 79.57 & 74.55 & 92.66 & 89.02 & 85.86 & 82.48 & 64.10 & 56.90 & 85.04 & 67.62 & 61.14 \\
    SA-SSD \cite{sassd_he} & 88.75 & 79.79 & 74.16 & \textbf{95.03} & \textbf{91.03} & 85.96 & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ \\
 %   VoTr \cite{votr_mao} & 89.90 & 82.09 & \textbf{79.14} & 94.03 & 90.34 & 86.14 & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ \\
    \hline
    PointRCNN \cite{pointrcnn_shi} & 86.96 & 75.64 & 70.70 & 92.13 & 87.39 & 82.72 & 74.96 & 58.82 & 52.53 & 82.56 & 67.24 & 60.28 \\
 %   Fast Point RCNN \cite{fastpointrcnn_chen} & 85.29 & 77.40 & 70.24 & 90.87 & 87.84 & 80.52 & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ \\
    PartA$^{2}$ \cite{parta2_shi} & 87.81 & 78.49 & 73.51 & 91.70 & 87.79 & 84.61 & 79.17 & 63.52 & 56.93 & 83.43 & 68.73 & 61.85 \\
    Point-GNN \cite{pointgnn_shi} & 88.33 & 79.47 & 72.29 & 93.11 & 89.17 & 83.90 & 78.60 & 63.48 & 57.08 & 81.17 & 67.28 & 59.67 \\
    PV-RCNN \cite{pvrcnn_shi} & 90.25 & 81.43 & 76.82 & \underline{94.98} & \underline{90.65} & 86.14 & 78.60 & 63.71 & 57.65 & 82.49 & 68.89 & 62.41 \\
    Voxel R-CNN \cite{voxelrcnn_deng} & \textbf{90.90} & 81.62 & 77.06 & 94.85 & 88.83 & 86.13 & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ \\
    PV-RCNN + SPG \cite{spg_xu} & \underline{90.64} & \underline{82.66} & 77.91 & 92.80 & 89.12 & 86.27 & 80.21 & 66.96 & 60.50 & 82.66 & 70.09 & 63.61 \\
    CT3D \cite{ct3d_sheng} & 87.83 & 81.77 & 77.16 & 92.36 & 88.83 & 84.07 & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ \\ 
    BtcDet \cite{btc_xu} & \underline{90.64} & \textbf{82.86} & \underline{78.09} & 92.81 & 89.34 & 84.55 & 82.81 & \textbf{68.68} & \textbf{61.81} & 84.48 & 71.76 & 64.70 \\
    PDV \cite{pdv_hu} & 90.43 & 81.86 & 77.36 & 94.56 & 90.48 & 86.23 & 83.04 & 67.81 & 60.46 & 85.54 & 71.31 & 64.40 \\
    \hline
    PC-RGNN \cite{pcrgnn_zhang} & 89.13 & 79.90 & 75.54 & 94.91 & 89.62 & \textbf{86.57} & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ \\
    SIENet \cite{sienet_li} & 88.22 & 81.71 & 77.22 & 92.38 & 88.65 & 86.03 & 83.00 & 67.61 & 60.09 & 84.64 & 71.21 & 64.61 \\
    \hline
    PG-RCNN (Ours) & 88.80	& 81.63 & 76.94	& 93.08	& 89.20 & 86.33 & \textbf{83.13}	& \underline{67.94}	& \underline{61.23}	& \textbf{86.40}	& \textbf{72.97}	& \textbf{64.89} \\
    \hline
  \end{tabular}
  }
\end{table*}

==> texts/table1.tex <==
\begin{table}[ht!]
 \caption{Comparison with state-of-the-art methods on the KITTI \textit{val} set. $^\dag$ denotes point completion approaches. $^\ddag$ denotes SIENet with baseline RPN.}
  % \caption{Comparison with state-of-the-art methods on the KITTI \textit{val} set. The results are evaluated with the Average Precision (AP) under 40 recall positions for moderate difficulties. The performances are retrieved from the publically released models. $^\dag$ denotes that the results are retrieved from the publication. $^\ddag$ is the case where SIENet uses the same backbone as ours.}
  \centering
  \label{table:kitti_val2}
  \resizebox{\linewidth}{!}{%
  \begin{tabular}{l||c|c|c c c}
    \hline
    \multirow{2}{*}{Method} &
    Param.&
    Latency&
    \multicolumn{3}{c}{3D AP$_{R40}$} \\
    % \cline{2-10}
    &(M) & (ms)& Car & Ped. & Cyc.  \\
    \hline
    SECOND \cite{second_yan}&5.33&59.9& 81.61 & 51.15 & 66.74 \\ % OpenPCDet
    PointPillars \cite{pointpillars_lang}&4.83&36.5& 78.41 & 51.42 & 62.93 \\ % OpenPCDet
    PointRCNN \cite{pointrcnn_shi}&4.04&171.5& 80.53 & 55.70 & 73.13\\ % OpenPCDet
 %   PartA$^2$ \cite{parta2_shi} &226& 80.29 & 66.37 & 75.33 \\ % OpenPCDet
    PC-RGNN$^\dag$ \cite{pcrgnn_zhang} & 21.43 & 152.4 & 81.43 & $-$  & $-$  \\ % paper
    PV-RCNN \cite{pvrcnn_shi}&13.12& 103.5& 84.39 & 54.51 & 70.38 \\ % OpenPCDet
    Voxel-RCNN \cite{voxelrcnn_deng}&7.59& 93.2&83.19 & $-$ & $-$ \\ % OpenPCDet
%    CT3D \cite{ct3d_sheng}& 92.85 & 85.82 & 83.46 & 65.73 & 58.56 & 53.04 & 91.99 & 71.60 & 67.34 \\
    SIENet$^\dag$ \cite{sienet_li} & 24.62 & 120.8 & \textbf{85.43} & $-$ & $-$ \\
    SIENet$^\ddag$ &24.40&118.3& 84.48 & $-$ & $-$ \\
    CT3D \cite{ct3d_sheng}&7.85&142.3& 84.97 & 55.57 & 71.88 \\
    PDV \cite{pdv_hu}&12.86&161.5& 85.05 & 57.41 & 75.95 \\
    % BtcDet$^{\dag}$ \cite{btc_xu}& 93.15 & 86.28 & 83.86 & 69.39 & 61.19 & 55.86 &91.45 & 74.70 & 70.08 \\
    % BtcDet$^{\dag}$ \cite{btc_xu}&&&&&&&& \\
    \hline
    PG-RCNN (Ours) & \textbf{2.76} & \textbf{59.0} & 85.09 & \textbf{60.88} & \textbf{76.05}\\
    \hline
\end{tabular}
}
\end{table}

==> texts/table3.tex <==
\begin{table*}[ht!]
  \caption{Comparison with state-of-the-art methods on the validation set of Waymo Open Dataset}
  \centering
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{l||c c c c |c c c c|c c c c}
    \hline
    \multirow{3}{*}{Method} &
    \multicolumn{4}{c|}{Vehicle} &
    \multicolumn{4}{c|}{Pedestrian} &
    \multicolumn{4}{c}{Cyclist}\\
    \cline{2-13}
    &
    \multicolumn{2}{c}{LEVEL\_1}&
    \multicolumn{2}{c|}{LEVEL\_2}&
    \multicolumn{2}{c}{LEVEL\_1}&
    \multicolumn{2}{c|}{LEVEL\_2}&
    \multicolumn{2}{c}{LEVEL\_1}&
    \multicolumn{2}{c}{LEVEL\_2}\\
    & mAP & mAPH & mAP & mAPH & mAP & mAPH & mAP & mAPH & mAP & mAPH & mAP & mAPH  \\
    \hline
    PV-RCNN$^\dag$ \cite{pvrcnn_shi} &75.29&74.61&66.75&	66.12&72.12&60.71&63.05&52.90&66.43&64.39&	63.97&62.00\\
    Voxel R-CNN$^\dag$ \cite{voxelrcnn_deng} &75.71	&75.22&67.29&66.85&77.81&71.53&69.17&63.37&	69.62&68.55&67.06&66.03\\
    \hline
    PG-RCNN (Ours) &\\
    \hline
\end{tabular}
}
\end{table*}
